3D Foundation Model-Based Loop Closing for Decentralized Collaborative SLAM

Decentralized Collaborative Simultaneous Localization And Mapping (C-SLAM) techniques often struggle to identify map overlaps due to significant viewpoint variations among robots. Motivated by recent advancements in 3D foundation models, which can register images despite large viewpoint differences, we propose a robust loop closing approach that leverages these models to establish inter-robot measurements. In contrast to resource-intensive methods requiring full 3D reconstruction within a centralized map, our approach integrates foundation models into existing SLAM pipelines, yielding scalable and robust multi-robot mapping. Our contributions include: (1) integrating 3D foundation models to reliably estimate relative poses from monocular image pairs within decentralized C-SLAM; (2) introducing robust outlier mitigation techniques critical to the use of these relative poses; and (3) developing specialized pose graph optimization formulations that efficiently resolve scale ambiguities. We evaluate our method against state-of-the-art approaches, demonstrating improvements in localization and mapping accuracy, alongside significant gains in computational and memory efficiency. These results highlight the potential of our approach for deployment in large-scale multi-robot scenarios.

==> figures/experimentation_figures.tex <==
%!TEX root = ../main.tex

%<*conf-pr>
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/conf_pr.pdf}
    \caption{Precision-Recall curves for various inlier/outlier detection techniques. MASt3R-based correspondences combined with the loop-to-odometry ratio yield the best performance.}
    \label{fig:conf-pr}
    \vspace{-5mm}
\end{figure}
%</conf-pr>

%<*conf-pg-boxplot>
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/conf_pg_boxplot.pdf}
    \caption{Translation errors for different confidence estimation methods and optimization techniques on the GrAco 6-robot
    dataset~\cite{zhuGRACOMultimodalDataset2023}. Our confidence measure based
    on the feature correspondence ratio significantly outperforms uniform confidence estimates, enabling even non-robust Levenberg–Marquardt
    optimization~\cite{f.dellaertetal.GeorgiaTechSmoothing} to yield accurate
    results—comparable to the robust Graduated Non-Convexity~\cite{yangGraduatedNonConvexityRobust2020b} solver.}
    \label{fig:conf-pg-boxplot}
\end{figure}
%</conf-pg-boxplot>

%<*ratios-results>
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/ratios_results.pdf}
    \caption{Impact of the correspondences ratio threshold on Average Translation Error (ATE) in pose graph optimization on the GrAco 6-robot dataset. Using ratio-based confidence yields consistently low ATE, even with less conservative thresholds, unlike uniform confidence. The dashed line shows the number of loop closures at different thresholds, where higher ratios lead to fewer closures.}
    \label{fig:ratios-results}
\end{figure}
%</ratios-results>

%<*scaling-init>
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/scaling_init_t_error.pdf}
    \caption{Translation errors for different registration methods with various loop closure scaling techniques. MASt3R combined with odometry-based scaling yields the best results, likely due to its higher scale consistency with visually similar inputs. In contrast, odometry-based scaling has little to no effect on other image matching methods.}
    \label{fig:scaling-init}
\end{figure}
%</scaling-init>

%<*sparse-kf-results>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/sparse_kf_results_independent_scales_lm.pdf}
    \caption{ Average Trajectory Error (ATE) versus keyframe distance, each registration technique is shown in a different color. Solid lines indicate the ATE with shaded regions representing standard deviation; dashed lines show the number of detected loop closures. Increasing keyframe distance reduces memory usage but typically degrades accuracy. Our approach maintains lower error, even with sparser keyframes.} \label{fig:sparse-kf}
    \vspace{-5mm}
\end{figure}
%</sparse-kf-results>

%<*sparse-kf-results-supp>
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{figures/sparse_kf_results_independent_scales_lm.pdf}
        \caption{With L2 Solver (Levenberg-Marquardt)}
        \label{fig:sparse-kf-lm}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{figures/sparse_kf_results_independent_scales_gnc.pdf}
        \caption{With Robust Solver (Graduated Non-Convexity)}
        \label{fig:sparse-kf-gnc}
    \end{subfigure}
    \caption{ATE vs. keyframe distance for different image matching techniques. Dashed lines indicate the number of loop closures. Increasing keyframe distance reduces memory usage but degrades accuracy in most methods. Our approach enables sparser, memory-efficient \gls{cslam} without sacrificing accuracy. While SuperPoint+SuperGlue is resilient to keyframe sparsity when using a robust solver, our method achieves similar performance with both solvers.}
    \label{fig:sparse-kf}
\end{figure*}
%</sparse-kf-results-supp>

%<*split-compute>
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/split_compute.pdf}
    \caption{Computational savings from two-stage MASt3R processing in C-SLAM. Splitting encoder and decoder processing reduces computation by avoiding redundant re-encoding of images with established loop closures. This is especially beneficial for onboard computers, where MASt3R processing is significantly more demanding than on a desktop server.
    }
    \label{fig:split-compute}
    \vspace{-5mm}
\end{figure}
%</split-compute>

%<*viz-graco>
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=\textwidth]{figures/viz_graco_ours.pdf}
        \caption{\gls{mold}}
        \label{fig:viz-graco-ours}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\columnwidth}
        \includegraphics[width=\textwidth]{figures/viz_graco_ss_lidar.pdf}
        \caption{Swarm-SLAM (LiDAR)}
        \label{fig:viz-graco-ss-lidar}
    \end{subfigure}
    \caption{Trajectory estimates of our approach on the GrAco 6-robot dataset compared to the LiDAR-based Swarm-SLAM solution.}
    \label{fig:viz-graco-all}
\end{figure}
%</viz-graco>

%<*viz-s3e>
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.495\columnwidth}
        \includegraphics[width=\columnwidth]{figures/viz_dormitory_ours.pdf}
        \caption{\gls{mold}}
        \label{fig:viz-square-ours}
    \end{subfigure}
    \begin{subfigure}[b]{0.505\columnwidth}
        \includegraphics[width=\columnwidth]{figures/ss_viz_graph_dorm.pdf}
        \caption{Swarm-SLAM LiDAR}
        \label{fig:viz-dormitory-ours}
    \end{subfigure}
    \caption{S3E Dormitory trajectory estimates with \gls{mold} versus Swarm-SLAM in LiDAR configuration.}
    \label{fig:viz-s3e-all}
    \vspace{-5mm}
\end{figure}
%</viz-s3e>


%<*s3e-table>
\begin{table*}[h]
    \vspace{4mm}
    \centering
    \caption{Average translation error (ATE), number of loop closures ($N$) and optimization time on S3E sequences.}
    \input{figures/table_results.tex}
    \label{tab:s3e}
\end{table*}
%</s3e-table>

%<*opt-vins-table>
\begin{table*}[t]
    \vspace{4mm}
    \centering
    \caption{Comparison of different pose graph optimization formulations with a VINS-Mono odometry backbone.}
    \input{figures/opt_results_table_vins.tex}
    \label{tab:graco-vins}
    \vspace{-5mm}
\end{table*}
%</opt-vins-table>

%<*opt-lio-table>
\begin{table*}[t]
    \vspace{4mm}
    \centering
    \caption{Comparison of different pose graph optimization formulations with a LIO odometry backbone.}
    \input{figures/opt_results_table_lio.tex}
    \label{tab:graco-lio}
    \vspace{-5mm}
\end{table*}
%</opt-lio-table>


==> figures/explanation_figures.tex <==
%!TEX root = ../main.tex
%<*system-overview>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/system-overview.pdf}
    \caption{System overview of the proposed \gls{mold} framework for decentralized \gls{cslam}. The figure illustrates the key components, highlighting how inter-robot loop closures are generated using a 3D foundation model, the multi-robot pose graph and loop scale optimization. Robots communicate with each other during place recognition, registration, and optimization, distributing tasks among neighboring robots to prevent duplicate processing.
    }
    \label{fig:mold-overview}
\end{figure}
%</system-overview>

%<*cslam-example>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/CSLAM-example.pdf}
    \caption{Illustration of the decentralized \acrshort{cslam} problem. Each robot independently explores an unknown environment, generating its own map. Upon meeting, the robots exchange data and compute inter-robot loop closures to register and eventually fuse their maps, thereby enhancing localization accuracy and enabling collaborative behaviors.}
    \label{fig:cslam-example}
\end{figure}
%</cslam-example>

%<*ratio-example>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/ratio-example.pdf}
    \caption{Example triplet of images used for inference, illustrating the ratio of correspondences between loop frames (in orange) and odometry frame pairs (in blue).}
    \label{fig:ratio-example}
\end{figure}
%</ratio-example>

%<*mast3r>
\begin{figure}
    \centering
    \includegraphics[width=0.92\columnwidth]{figures/mast3r.pdf}
    \caption{Illustration of our inference pipeline, highlighting the inter-robot processing of loop closures.}
    \label{fig:mast3r}
    \vspace{-5mm}
\end{figure}
%</mast3r>

%<*viz-registration>
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/resgistrationexample.pdf}
    \caption{Successful registration using MASt3R with minimal image overlap, illustrating its robustness in handling challenging loop closures.}
    \label{fig:registration-example}
\end{figure}
%</viz-registration>

%<*factor-graphs>
\begin{figure}
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/mold-factor-graph.pdf}
        \caption{Base Multi-Robot Factor Graph}
        \label{fig:factor-graph-base}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/mold-factor-graph-ind.pdf}
        \caption{Independent Scales Multi-Robot Factor Graph}
        \label{fig:factor-graph-independent-scales}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/mold-factor-graph-smoothed.pdf}
        \caption{Smoothed Scales Multi-Robot Factor Graph}
        \label{fig:factor-graph-smoothed-scales}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/mold-factor-graph-single.pdf}
        \caption{Single Scale Multi-Robot Factor Graph}
        \label{fig:factor-graph-single-scale}
    \end{subfigure}
    \caption{Illustrations of the proposed multi-robot factor graph formulations for pose graph optimization with or without scale estimation. In the figures, circles represent variable nodes (e.g., poses or scales), while squares represent factor nodes, which define relationships between the variables. Formulation (a) is basic pose graph optimization. Formulation (b) introduces separate variables for scale optimization. Formulation (c) add smoothing factors to model the correlation between scale variables. Formulation (d) assumes that all loop closures share the same scale. In our experiments, we compare the proposed formulation and conclude that (b) and (c) offer the most accurate solutions.}
    \label{fig:factor-graphs}
\end{figure}
%</factor-graphs>


==> figures/opt_results_table_lio.tex <==
\begin{tabular}{cccccccccc}
\toprule
 & \multicolumn{3}{c}{GT Scale} & \multicolumn{3}{c}{MASt3R Scale} & \multicolumn{3}{c}{Odometry Scale} \\
 & ATE (m) & Onb.(s) & Srv.(s) & ATE (m) & Onb.(s) & Srv.(s) & ATE (m) & Onb.(s) & Srv.(s) \\
\midrule
LM & 2.75 $\pm$ 1.36 & 1.44 & 0.29 & 10.36 $\pm$ 3.65 & 1.44 & 0.30 & 6.90 $\pm$ 3.95 & 1.51 & 0.30 \\
GNC & 2.73 $\pm$ 1.36 & 29.61 & 9.58 & 9.25 $\pm$ 2.98 & 29.12 & 9.56 & 2.95 $\pm$ 1.32 & 30.71 & 9.89 \\
%OneS-LM & 3.06 $\pm$ 1.32 & 1.46 & 0.30 & 4.47 $\pm$ 2.57 & 1.44 & 0.30 & 10.15 $\pm$ 3.63 & 1.43 & 0.31 \\
%OneS-GNC & 2.97 $\pm$ 1.28 & 29.81 & 9.74 & 3.63 $\pm$ 1.75 & 28.95 & 9.54 & 6.53 $\pm$ 2.21 & 31.78 & 10.47 \\
IS-LM & 3.45 $\pm$ 2.03 & 3.16 & 0.74 & 3.14 $\pm$ 1.80 & 2.83 & 0.66 & 3.41 $\pm$ 1.96 & 3.01 & 0.70 \\
IS-GNC & 3.45 $\pm$ 2.00 & 93.70 & 26.45 & 3.12 $\pm$ 1.77 & 87.59 & 24.63 & 3.40 $\pm$ 1.94 & 94.17 & 26.31 \\
SS-LM & 2.92 $\pm$ 1.93 & 4.06 & 0.95 & 3.29 $\pm$ 1.94 & 3.42 & 0.80 & 3.11 $\pm$ 1.81 & 3.85 & 0.84 \\
SS-GNC & 2.93 $\pm$ 1.90 & 156.52 & 41.42 & 3.23 $\pm$ 1.92 & 139.69 & 37.32 & 13.89 $\pm$ 11.23 & 342.36 & 89.20 \\

\end{tabular}

==> figures/opt_results_table_vins.tex <==
\begin{tabular}{cccccccccc}
\toprule
 & \multicolumn{3}{c}{GT Scale} & \multicolumn{3}{c}{MASt3R Scale} & \multicolumn{3}{c}{Odometry Scale} \\
 & ATE (m) & Onb.(s) & Srv.(s) & ATE (m) & Onb.(s) & Srv.(s) & ATE (m) & Onb.(s) & Srv.(s) \\
\midrule
LM & 4.76 $\pm$ 4.50 & 1.60 & 0.33 & 39.93 $\pm$ 44.43 & 3.63 & 0.91 & 39.59 $\pm$ 45.68 & 3.27 & 0.79 \\
GNC & 4.89 $\pm$ 4.51 & 31.09 & 10.28 & 11.98 $\pm$ 5.21 & 32.93 & 10.49 & 5.56 $\pm$ 4.07 & 35.86 & 11.78 \\
%OneS-LM & 12.35 $\pm$ 13.50 & 1.55 & 0.34 & 38.55 $\pm$ 44.71 & 3.99 & 1.10 & 40.35 $\pm$ 44.51 & 3.77 & 0.92 \\
%OneS-GNC & 12.42 $\pm$ 13.53 & 32.07 & 10.64 & 4.91 $\pm$ 3.31 & 34.54 & 11.86 & 10.14 $\pm$ 5.13 & 37.17 & 12.12 \\
IS-LM & 6.99 $\pm$ 6.47 & 3.27 & 0.79 & 7.11 $\pm$ 6.81 & 3.24 & 0.78 & 7.89 $\pm$ 7.01 & 3.49 & 0.87 \\
IS-GNC & 6.34 $\pm$ 6.51 & 104.21 & 29.65 & 6.40 $\pm$ 6.82 & 96.54 & 27.38 & 7.86 $\pm$ 7.01 & 112.94 & 31.98 \\
SS-LM & 7.43 $\pm$ 6.93 & 3.89 & 0.94 & 8.23 $\pm$ 7.34 & 3.50 & 0.82 & 7.42 $\pm$ 7.06 & 3.95 & 0.94 \\
SS-GNC & 7.45 $\pm$ 7.06 & 166.24 & 45.99 & 91.50 $\pm$ 59.82 & 296.27 & 85.31 & 58.94 $\pm$ 62.61 & 305.20 & 85.38 \\

\end{tabular}

==> figures/table_results.tex <==
\addtolength{\tabcolsep}{-0.5em}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
 &  & \multicolumn{3}{c}{Campus} & \multicolumn{3}{c}{Teaching} & \multicolumn{3}{c}{Square} & \multicolumn{3}{c}{Dormitory}\\
 &  & ATE (m) & $N$ & Time (s) & ATE (m) & $N$ & Time (s) & ATE (m) & $N$ & Time (s) & ATE (m) & $N$ & Time (s) \\
\midrule
\multirow[t]{2}{*}{\multirow{2}{*}{\gls{mold}}} & GNC & 19.25 $\pm$ 6.81 & 1122 & 27.45 & 2.40 $\pm$ 0.76 & 2274 & 41.58 & 9.53 $\pm$ 3.87 & 226 & 9.25 & 46.00 $\pm$ 30.36 & 175 & 34.79 \\
 & IS-LM & 5.50 $\pm$ 2.16 & 1122 & 2.46 & 1.87 $\pm$ 0.65 & 2273 & 3.46 & 5.64 $\pm$ 2.46 & 226 & 1.41 & 3.84 $\pm$ 1.35 & 175 & 1.50 \\
 \multirow[t]{1}{*}{\multirow{1}{*}{\centering \textit{Monocular loop closures}}} & SS-LM & \textbf{5.41} $\pm$ \textbf{2.13} & 1122 & 1.82 & \textbf{1.84 $\pm$ 0.67} & 2273 & 4.74 & \textbf{5.07 $\pm$ 2.56} & 226 & 1.63 & \textbf{2.41 $\pm$ 0.99} & 175 & 11.05 \\
\cline{1-14}
\multirow[t]{2}{*}{\multirow{2}{*}{\centering Swarm-SLAM}} & RBCD & 9.41 $\pm$ 7.59 & 29 & 286.63 & 3.59 $\pm$ 1.56 & 110 & 143.31 & 113.58 $\pm$ 80.99 & 6 & 120.33 & 7.41 $\pm$ 5.32 & 226 & 147.80 \\
 & GNC & 10.50 $\pm$ 9.47 & 29 & 21.38 & 3.69 $\pm$ 1.52 & 110 & 13.97 & 164.83 $\pm$ 99.39 & 6 & 36.45 & 10.18 $\pm$ 5.47 & 226 & 26.14 \\
 \multirow[t]{1}{*}{\multirow{1}{*}{\centering \textit{LiDAR loop closures}}} & LM & 10.21 $\pm$ 8.97 & 29 & 1.23 & 3.85 $\pm$ 1.63 & 110 & 0.99 & 165.94 $\pm$ 98.98 & 6 & 1.73 & 8.34 $\pm$ 4.82 & 226 & 4.02 \\
\cline{1-14}
\multirow[t]{2}{*}{\multirow{2}{*}{\centering Swarm-SLAM}} & RBCD & 6.79 $\pm$ 7.08 & 16 & 744.65 & 2.23 $\pm$ 0.94 & 27 & 840.53 & 42.97 $\pm$ 25.27 & 7 & 2.46 &  & \xmark &  \\
 & GNC & 6.56 $\pm$ 7.07 & 16 & 48.64 & 2.25 $\pm$ 1.15 & 27 & 23.85 & 9.73 $\pm$ 6.67 & 7 & 15.34 &  & \xmark &  \\
\multirow[t]{1}{*}{\multirow{1}{*}{\centering \textit{Stereo loop closures}}} & LM & 6.56 $\pm$ 7.07 & 16 & 2.90 & 2.20 $\pm$ 1.05 & 27 & 3.91 & 33.37 $\pm$ 22.98 & 7 & 1.27 &  & \xmark  &  \\
\cline{1-14}

\end{tabular}

==> sections/supplemental_material.tex <==
\ExecuteMetaData[figures/experimentation_figures.tex]{scaling-init}

Using the loop closure inliers from our set of image pairs, we compared different scale initialization techniques, as shown in~\cref{fig:scaling-init}. We evaluated ground truth scaling, the direct approach (which uses the raw output of MASt3R), and scaling based on odometry estimates (see~\cref{eq:scaleinit}). Additionally, we compared these results with relative poses obtained using SuperPoint+SuperGlue and OpenCV (which implements Nister's method~\cite{nisterEfficientSolutionFivepoint2004} with ORB~\cite{rubleeORBEfficientAlternative2011} features and descriptors) to assess whether our scale initialization method would also benefit those approaches.

The results in~\cref{fig:scaling-init} demonstrate that our approach significantly reduces translation error for data-driven MASt3R, whereas the same improvement was not observed with the other methods. This may be explained by MASt3R's ability to output 3D point maps that are scale-consistent within a given image domain or environment. However, the mean translation error remains above 2 meters, which is high for accurate pose graph optimization. Therefore, further refinement of the scale during pose graph optimization is necessary.


\ExecuteMetaData[figures/experimentation_figures.tex]{conf-pg-boxplot}

In the following experiments, we evaluate the full pose graph solution involving all six robots from the GrAco sequence. Based on the previously mentioned feature correspondences ratio, we mapped it to a confidence metric (see~\cref{eq:confidence}), which we used to weight the inter-robot loop closures during pose graph optimization.

\cref{fig:conf-pg-boxplot} compares translation errors based on different confidence estimation methods for inter-robot loop closures and optimization techniques during map optimization. Our proposed confidence estimation, derived from the feature correspondences ratio, significantly outperforms the commonly used uniform confidence estimates, which are often adopted due to the difficulty of accurately estimating confidence~\cite{lajoieSwarmSLAMSparseDecentralized2024}. The figure illustrates that, even with the non-robust Levenberg-Marquardt optimization~\cite{f.dellaertetal.GeorgiaTechSmoothing}, our method produces accurate results, whereas uniform confidence estimates lead to failure. Moreover, our approach achieves results comparable to the computationally expensive Graduated Non-Convexity solver~\cite{yangGraduatedNonConvexityRobust2020b}.


\ExecuteMetaData[figures/experimentation_figures.tex]{ratios-results}

In~\cref{fig:ratios-results}, we compare different correspondences ratios threshold, used for outlier rejection, with the Average Translation Error (ATE), using the LM solver with either uniform confidence or correspondences ratio-based confidence. The dashed line represents the number of loop closures at various threshold levels. A higher ratio results in a more conservative solution, yielding fewer loop closures. Notably, with our ratio-based confidence estimation, the ATE remains low even with less conservative thresholds, showing that this method simplifies parameter tuning by effectively minimizing the influence of outliers without relying on a robust solver. However, if the ratio threshold is set too conservatively, insufficient inter-robot loop closures are included, leading to decreased accuracy or failure to merge the maps.




We also observed that while our odometry-based scaling initialization sometimes improved results, it could also lead to worse performance. This suggests that our assumption—that MASt3R yields similar relative pose scales for odometry images and loop closure images—may not always hold, and altering initial estimates in local solvers can have a significant impact. Therefore, using the raw output directly and relying solely on scale optimization may offer equally good results.


Overall, these findings demonstrate the robustness and flexibility of our approach. Even with initial scale inaccuracies, the system can adapt and optimize effectively without requiring computationally expensive methods. Our independent and smoothed scale formulations consistently provide accurate results while maintaining efficient performance.

